UniTE: A Survey and Unified Pipeline for Pre-training Spatiotemporal Trajectory Embeddings

Spatiotemporal trajectories are sequences of timestamped locations, which enable a variety of analyses that in turn enable important real-world applications. It is common to map trajectories to vectors, called embeddings, before subsequent analyses. Thus, the qualities of embeddings are very important. Methods for pre-training embeddings, which leverage unlabeled trajectories for training universal embeddings, have shown promising applicability across different tasks, thus attracting considerable interest. However, research progress on this topic faces two key challenges: a lack of a comprehensive overview of existing methods, resulting in several related methods not being well-recognized, and the absence of a unified pipeline, complicating the development of new methods and the analysis of methods. We present UniTE, a survey and a unified pipeline for this domain. In doing so, we present a comprehensive list of existing methods for pre-training trajectory embeddings, which includes methods that either explicitly or implicitly employ pre-training techniques. Further, we present a unified and modular pipeline with publicly available underlying code, simplifying the process of constructing and evaluating methods for pre-training trajectory embeddings. Additionally, we contribute a selection of experimental results using the proposed pipeline on real-world datasets. Implementation of the pipeline is publicly available at https://github.com/Logan-Lin/UniTE.

==> plot/finetune-scalability.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ftScaleAcc

\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ftScaleRec

\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ftScaleF

==> plot/pretrain-scalability.tex <==
\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ptScaleAcc1

\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ptScaleAcc5

\pgfplotstableread[row sep=\\,col sep=&]{
method & 20 & 40 & 60 & 80 & 100 \\
CAESC & 83.720 & 77.425 & 72.471 & 77.425 & 72.471 \\
}\ptScaleAcc10

==> table/classification_old.tex <==
\begin{threeparttable}
%\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
    Datasets & \multicolumn{4}{c|}{Chengdu} & \multicolumn{4}{c}{Porto} \\
    \midrule
    Metric & Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) & 
    Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) \\
    \midrule
	CAESC w/o finetune & 0.55$\pm$0.28 & 1.43$\pm$0.69 & 0.5$\pm$0.27 & 0.4$\pm$0.23 & 1.31$\pm$0.26 & 4.75$\pm$0.59 & 0.85$\pm$0.09 & 0.24$\pm$0.09 \\
    CAESC w/o pretrain & 0.04$\pm$0.03 & 0.17$\pm$0.06 & 0.02$\pm$0.02 & 0.0$\pm$0.0 & 3.48$\pm$1.0 & 11.7$\pm$2.91 & 2.83$\pm$0.88 & 1.65$\pm$0.65\\
    CAESC  & 0.03$\pm$0.01 & 0.15$\pm$0.03 & 0.02$\pm$0.0 & 0.0$\pm$0.0 & 2.77$\pm$0.76 & 9.81$\pm$2.05 & 2.03$\pm$0.65 & 1.06$\pm$0.5\\
    GCM w/o finetune & 9.53$\pm$0.13 & 11.14$\pm$0.07 & 7.46$\pm$0.12 & 6.87$\pm$0.13 & 5.07$\pm$0.15 & 14.63$\pm$0.21 & 4.53$\pm$0.19 & 3.39$\pm$0.16\\
    GCM w/o pretrain & 11.09$\pm$0.17 & 12.03$\pm$0.08 & 8.57$\pm$0.15 & 7.9$\pm$0.11 & 4.94$\pm$0.22 & 14.71$\pm$0.58 & 4.3$\pm$0.16 & 3.17$\pm$0.28\\
    GCM & 10.15$\pm$0.19 & 11.67$\pm$0.06 & 8.15$\pm$0.09 & 7.53$\pm$0.1 & 5.18$\pm$0.22 & 15.33$\pm$0.39 & 4.57$\pm$0.18 & 3.22$\pm$0.21\\
    GM-VSAE w/o finetune & 11.96$\pm$0.08 & 12.32$\pm$0.03 & 9.84$\pm$0.05 & 9.1$\pm$0.05 & 4.88$\pm$0.11 & 15.55$\pm$0.23 & 4.25$\pm$0.15 & 2.59$\pm$0.18\\
    GM-VSAE w/o pretrain & 11.99$\pm$0.2 & 12.21$\pm$0.02 & 9.05$\pm$0.14 & 8.21$\pm$0.12 & 5.69$\pm$0.15 & 16.84$\pm$0.34 & 5.08$\pm$0.19 & 3.69$\pm$0.12 \\
    GM-VSAE & 12.17$\pm$0.03 & 12.33$\pm$0.04 & 9.65$\pm$0.04 & 8.79$\pm$0.06  & 5.72$\pm$0.22 & 17.32$\pm$0.38 & 4.98$\pm$0.28 & 3.54$\pm$0.27\\
    PreCLN w/o finetune &11.54$\pm$0.25 & 12.36$\pm$0.07 & 9.49$\pm$0.09 & 8.81$\pm$0.11 & 4.48$\pm$0.29 & 12.39$\pm$0.43 & 4.02$\pm$0.13 & 3.20$\pm$0.21\\
    PreCLN w/o pretrain & 6.65$\pm$0.08 & 7.97$\pm$0.07 & 5.48$\pm$0.10& 5.36$\pm$0.09 & 2.06$\pm$0.07 & 4.97$\pm$0.33 & 1.04$\pm$0.26 & 0.95$\pm$0.17 \\
    PreCLN & 6.69$\pm$0.12 & 8.12$\pm$0.17 & 5.97$\pm$0.20 & 5.67$\pm$0.22 & 1.96$\pm$0.24 & 5.37$\pm$0.52 & 1.17$\pm$0.26 & 1.22$\pm$0.33 \\
    START w/o finetune & 11.63$\pm$0.11 & 12.42$\pm$0.04 & 9.59$\pm$0.07 & 8.97$\pm$0.11 & 4.52$\pm$0.16 & 13.66$\pm$0.34 & 4.13$\pm$0.16 & 3.12$\pm$0.22 \\
    START w/o pretrain  & 7.65$\pm$3.32 & 9.95$\pm$3.35 & 6.51$\pm$2.64 & 6.07$\pm$2.5 & 6.18$\pm$0.17 & 19.63$\pm$0.28 & 5.46$\pm$0.28 & 3.8$\pm$0.35 \\
    START & 7.09$\pm$1.57 & 10.13$\pm$1.22 & 6.28$\pm$1.28 & 5.92$\pm$1.26 & 6.34$\pm$0.16 & 19.88$\pm$0.33 & 5.61$\pm$0.21 & 3.79$\pm$0.23\\
    TremBR w/o finetune & 11.17$\pm$0.15 & 12.08$\pm$0.07 & 8.76$\pm$0.09 & 8.1$\pm$0.08 & 4.89$\pm$0.13 & 14.58$\pm$0.1 & 4.3$\pm$0.16 & 2.79$\pm$0.38\\
    TremBR w/o pretrain & 11.33$\pm$0.14 & 12.05$\pm$0.05 & 8.34$\pm$0.09 & 7.59$\pm$0.06 & 6.04$\pm$0.21 & 17.85$\pm$0.28 & 5.25$\pm$0.2 & 3.73$\pm$0.29\\
    TremBR & 11.55$\pm$0.04 & 12.22$\pm$0.03 & 8.89$\pm$0.04 & 8.16$\pm$0.03 & 5.65$\pm$0.24 & 16.86$\pm$0.46 & 4.92$\pm$0.29 & 3.65$\pm$0.11\\
    TrajectorySim w/o finetune & 8.60$\pm$0.11 & 10.65$\pm$0.04 & 6.64$\pm$0.05 & 6.34$\pm$0.05 & 2.55$\pm$0.11 & 9.20$\pm$0.13 & 2.07$\pm$0.11 & 1.31$\pm$0.08\\
    TrajectorySim w/o pretrain & 9.66$\pm$0.18 & 11.10$\pm$0.08 & 7.42$\pm$0.12 & 7.12$\pm$0.10 & 2.79$\pm$0.15 & 10.39$\pm$0.28 & 2.31$\pm$0.11 & 1.34$\pm$0.05\\
    TrajectorySim  & 9.70$\pm$0.13 & 11.24$\pm$0.07 & 7.45$\pm$0.10 & 7.13$\pm$0.11 & 3.02$\pm$0.06 & 10.54$\pm$0.23 & 2.51$\pm$0.07 & 1.65$\pm$0.12\\
    t2vec w/o finetune & 9.67$\pm$0.08 & 11.42$\pm$0.05 & 7.18$\pm$0.06 & 6.48$\pm$0.05 & 5.39$\pm$0.10 & 16.47$\pm$0.21 & 4.71$\pm$0.08 & 3.43$\pm$0.14\\
    t2vec w/o pretrain & 11.97$\pm$0.05 & 12.25$\pm$0.03 & 9.45$\pm$0.06 & 8.65$\pm$0.04 & 5.36$\pm$0.14 & 16.55$\pm$0.14 & 4.70$\pm$0.18 & 3.23$\pm$0.30\\
    t2vec  & 11.71$\pm$0.04 & 12.23$\pm$0.02 & 8.85$\pm$0.08 & 8.11$\pm$0.05 & 5.74$\pm$0.11 & 16.91$\pm$0.21 & 5.08$\pm$0.11 & 3.75$\pm$0.18\\
    RobustDAA w/o finetune & 0.03$\pm$0.01 & 0.13$\pm$0.01 & 0.01$\pm$0.0 & 0.0$\pm$0.0 & 0.84$\pm$0.03 & 3.15$\pm$0.20 & 0.37$\pm$0.04 & 0.02$\pm$0.01\\
    RobustDAA w/o pretrain & 0.28$\pm$0.08 & 0.54$\pm$0.08 & 0.26$\pm$0.09 & 0.27$\pm$0.09 & 0.67$\pm$0.08 & 2.73$\pm$0.08 & 0.35$\pm$0.03 & 0.10$\pm$0.03\\
    RobustDAA  & 0.04$\pm$0.01 & 0.16$\pm$0.02 & 0.01$\pm$0.0 & 0.0$\pm$0.0 & 0.98$\pm$0.04 & 3.55$\pm$0.20 & 0.46$\pm$0.03 & 0.07$\pm$0.03\\
    LightPath w/o finetune & 2.18$\pm$0.13 & 4.24$\pm$0.17 & 1.89$\pm$0.09 & 1.74$\pm$0.06 & 4.76$\pm$0.16 & 14.4$\pm$0.11 & 4.34$\pm$0.1 & 2.91$\pm$0.15 \\
    LightPath w/o pretrain & 0.03$\pm$0.0 & 0.17$\pm$0.06 & 0.01$\pm$0.0 & 0.0$\pm$0.0 & 1.04$\pm$0.06 & 3.81$\pm$0.15 & 0.57$\pm$0.04 & 0.08$\pm$0.03 \\
    LightPath &0.97$\pm$0.27 & 2.19$\pm$0.64 & 0.91$\pm$0.17 & 0.78$\pm$0.12 & 0.98$\pm$0.25 & 3.56$\pm$0.45 & 0.54$\pm$0.08 & 0.07$\pm$0.04 \\
    \bottomrule
    \end{tabular}
%}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}

==> table/dataset-statistics.tex <==
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|ccc}
  \toprule
  Dataset & Chengdu & Porto \\
  \midrule
  Time span & 10.01--11.30, 2018 & 07.01--09.01, 2013 \\
  Longitude scope & 104.04300$\sim$104.12654 & -8.65200$\sim$-8.57801 \\
  Latitude scope & 30.65523$\sim$30.72699 & 41.14201$\sim$41.17399 \\
  Number of road segments & 2,505 & 2,225 \\
  Number of trajectories & 121,394 & 55,120  \\
  Number of points & 3,032,212 & 1,482,751  \\
  \bottomrule
\end{tabular}
}


==> table/destination_old.tex <==
\begin{threeparttable}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|cccc|cccc}
    \toprule
    Datasets & \multicolumn{4}{c|}{Chengdu} & \multicolumn{4}{c}{Porto} \\
    \midrule
    Metric & Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) & 
    Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) \\
    \midrule
    CAESC w/o finetune & 18.55$\pm$0.7 & 50.35$\pm$1.37 & 4.73$\pm$0.82 & 3.23$\pm$0.63 & 15.99$\pm$1.33 & 36.19$\pm$2.51 & 1.75$\pm$0.31 & 1.04$\pm$0.22\\
    CAESC w/o pretrain & 24.38$\pm$4.31 & 60.5$\pm$5.38 & 7.07$\pm$1.86 & 5.22$\pm$1.77 & 34.2$\pm$3.56 & 67.22$\pm$5.95 & 8.91$\pm$3.16 & 7.7$\pm$3.23\\
    CAESC  & 16.71$\pm$2.28 & 43.17$\pm$5.66 & 2.59$\pm$0.98 & 1.43$\pm$0.68 & 28.74$\pm$2.22 & 58.29$\pm$4.12 & 4.71$\pm$0.93 & 3.46$\pm$0.96 \\
    GCM w/o finetune & 53.73$\pm$0.3 & 86.56$\pm$0.21 & 22.45$\pm$0.83 & 20.85$\pm$0.85 & 33.43$\pm$0.41 & 66.74$\pm$0.41 & 8.16$\pm$0.26 & 7.36$\pm$0.34\\
    GCM w/o pretrain & 54.64$\pm$0.38 & 87.59$\pm$0.23 & 22.79$\pm$1.12 & 20.96$\pm$0.99 & 34.29$\pm$0.26 & 68.05$\pm$0.14 & 8.61$\pm$0.44 & 7.61$\pm$0.55\\
    GCM & 54.88$\pm$0.27 & 87.59$\pm$0.11 & 23.03$\pm$0.45 & 21.21$\pm$0.52 & 34.43$\pm$0.47 & 68.51$\pm$0.26 & 8.95$\pm$0.36 & 8.05$\pm$0.44 \\
    GM-VSAE w/o finetune & 31.85$\pm$0.4 & 70.07$\pm$0.28 & 15.04$\pm$1.69 & 13.85$\pm$1.73 & 24.43$\pm$0.3 & 49.36$\pm$0.21 & 6.24$\pm$0.26 & 5.89$\pm$0.19\\
    GM-VSAE w/o pretrain & 38.96$\pm$0.63 & 80.82$\pm$0.73 & 18.67$\pm$0.68 & 16.53$\pm$0.96 & 43.76$\pm$0.22 & 79.41$\pm$0.27 & 14.73$\pm$0.21 & 13.82$\pm$0.42\\
    GM-VSAE & 39.25$\pm$0.24 & 80.67$\pm$0.16 & 18.91$\pm$0.52 & 16.96$\pm$0.73 & 43.7$\pm$0.36 & 79.04$\pm$0.16 & 14.68$\pm$0.26 & 13.69$\pm$0.35\\
    PreCLN w/o finetune & 12.48$\pm$0.2 & 31.92$\pm$0.12 & 2.26$\pm$1.02 & 2.09$\pm$1.02 & 9.58$\pm$0.19 & 24.79$\pm$0.29 & 0.62$\pm$0.01 & 0.34$\pm$0.02\\
    PreCLN w/o pretrain & 53.06$\pm$0.51 & 87.63$\pm$0.39 & 20.33$\pm$0.59 & 18.03$\pm$0.73 & 37.35$\pm$0.19 & 73.14$\pm$0.12 & 9.96$\pm$0.23 & 8.66$\pm$0.24\\
    PreCLN & 48.45$\pm$1.24 & 83.9$\pm$1.41 & 14.55$\pm$1.63 & 11.58$\pm$1.54 & 36.5$\pm$0.28 & 72.0$\pm$0.5 & 8.99$\pm$0.13 & 7.46$\pm$0.18 \\
    START w/o finetune & 47.21$\pm$0.26 & 79.72$\pm$0.25 & 18.31$\pm$1.29 & 17.13$\pm$1.61 & 28.92$\pm$0.19 & 59.12$\pm$0.27 & 6.35$\pm$0.17 & 5.63$\pm$0.31\\
    START w/o pretrain & 55.14$\pm$1.91 & 87.83$\pm$1.14 & 21.46$\pm$3.23 & 19.14$\pm$3.73 & 36.13$\pm$0.69 & 71.33$\pm$0.94 & 9.17$\pm$0.59 & 7.63$\pm$0.64\\
    START & 55.28$\pm$0.81 & 86.53$\pm$2.5 & 23.81$\pm$3.7 & 21.84$\pm$4.44 & 36.87$\pm$0.33 & 72.96$\pm$0.31 & 9.96$\pm$0.41 & 8.41$\pm$0.4\\
    TremBR w/o finetune & 22.44$\pm$0.63 & 48.91$\pm$1.16 & 3.4$\pm$0.78 & 2.56$\pm$0.72 & 4.89$\pm$0.46 & 13.68$\pm$0.45 & 0.14$\pm$0.02 & 0.03$\pm$0.02\\
    TremBR w/o pretrain & 57.86$\pm$0.24 & 90.27$\pm$0.18 & 25.64$\pm$0.3 & 23.87$\pm$0.24 & 38.5$\pm$0.52 & 75.31$\pm$0.31 & 11.03$\pm$0.4 & 9.5$\pm$0.53\\
    TremBR & 56.09$\pm$0.19 & 88.4$\pm$0.27 & 23.88$\pm$0.6 & 22.06$\pm$0.67 & 38.14$\pm$0.16 & 74.16$\pm$0.31 & 10.14$\pm$0.24 & 8.6$\pm$0.26\\
    TrajectorySim w/o finetune & 30.42$\pm$0.31 & 57.10$\pm$0.30 & 8.33$\pm$0.83 & 8.29$\pm$0.99 & 19.42$\pm$0.27 & 43.07$\pm$0.28 & 2.60$\pm$0.10 & 2.22$\pm$0.10\\
    TrajectorySim w/o pretrain & 34.22$\pm$0.23 & 60.20$\pm$0.32 & 10.93$\pm$0.32 & 11.29$\pm$0.19 & 22.90$\pm$0.37 & 49.23$\pm$0.21 & 3.49$\pm$0.13 & 3.02$\pm$0.23\\
    TrajectorySim & 33.48$\pm$0.35 & 60.32$\pm$0.26 & 9.30$\pm$0.57 & 9.51$\pm$0.68 & 22.36$\pm$0.08 & 48.23$\pm$0.20 & 3.25$\pm$0.12 & 2.77$\pm$0.12\\
    t2vec w/o finetune & 54.47$\pm$0.28 & 86.80$\pm$0.17 & 24.41$\pm$0.98 & 22.84$\pm$1.13 & 37.81$\pm$0.26 & 72.82$\pm$0.20 & 10.27$\pm$0.25 & 9.44$\pm$0.28\\
    t2vec w/o pretrain & 55.67$\pm$0.21 & 87.71$\pm$0.24 & 24.96$\pm$0.70 & 23.29$\pm$0.77 & 38.14$\pm$0.25 & 73.76$\pm$0.27 & 10.70$\pm$0.49 & 9.29$\pm$0.67\\
    t2vec & 55.63$\pm$0.29 & 88.16$\pm$0.08 & 24.25$\pm$0.97 & 22.15$\pm$1.17 & 38.71$\pm$0.29 & 74.35$\pm$0.50 & 10.83$\pm$0.28 & 9.77$\pm$0.17\\
    RobustDAA w/o finetune & 5.84$\pm$0.03 & 15.74$\pm$2.41 & 0.11$\pm$0.001 & 0.01$\pm$0.002 & 4.88$\pm$0.07 & 14.27$\pm$0.17 & 0.21$\pm$0.01 & 0.04$\pm$0.004\\
    RobustDAA w/o pretrain & 8.13$\pm$0.62 & 20.10$\pm$1.87 & 0.50$\pm$0.21 & 0.42$\pm$0.21 & 5.54$\pm$0.13 & 14.81$\pm$1.05 & 0.31$\pm$0.05 & 0.22$\pm$0.05\\
    RobustDAA & 5.84$\pm$0.06 & 16.59$\pm$0.98 & 0.11$\pm$0.001 & 0.01$\pm$0.002 & 5.76$\pm$0.22 & 16.77$\pm$0.36 & 0.31$\pm$0.05 & 0.15$\pm$0.05\\
    trajectory2vec w/o finetune & 26.57$\pm$0.28 & 53.52$\pm$0.12 & 3.99$\pm$0.28 & 3.66$\pm$0.09 & 8.25$\pm$0.21 & 21.17$\pm$0.23 & 0.46$\pm$0.03 & 0.22$\pm$0.02\\
    trajectory2vec w/o pretrain & 29.35$\pm$1.43 & 56.97$\pm$1.68 & 4.68$\pm$0.37 & 4.15$\pm$0.35 & 4.92$\pm$0.10 & 13.50$\pm$0.25 & 0.14$\pm$0.01 & 0.03$\pm$0.01\\
    trajectory2vec & 36.25$\pm$1.20 & 64.99$\pm$1.59 & 7.55$\pm$1.02 & 6.99$\pm$1.03 & 6.07$\pm$1.72 & 15.96$\pm$4.63 & 0.39$\pm$0.05 & 0.16$\pm$0.05\\
    DTC w/o finetune & 6.56$\pm$0.66 & 16.86$\pm$0.55 & 0.13$\pm$0.02 & 0.03$\pm$0.01 & 4.02$\pm$1.16 & 10.29$\pm$2.65 & 0.12$\pm$0.00 & 0.01$\pm$0.00\\
    DTC w/o pretrain & 55.43$\pm$0.27 & 87.87$\pm$0.25 & 23.56$\pm$1.10 & 21.40$\pm$1.18 & 38.26$\pm$0.28 & 73.72$\pm$0.18 & 10.53$\pm$0.19 & 8.84$\pm$0.13\\
    DTC & 54.69$\pm$0.36 & 86.44$\pm$0.30 & 23.31$\pm$0.42 & 21.27$\pm$0.49 & 36.02$\pm$0.14 & 70.86$\pm$0.41 & 8.90$\pm$0.22 & 7.87$\pm$0.13\\
    LightPath w/o finetune & 51.0$\pm$0.20 & 84.11$\pm$0.23 & 18.62$\pm$0.59 & 16.72$\pm$0.64 & 31.48$\pm$0.11 & 63.55$\pm$0.09 & 7.16$\pm$0.23 & 6.36$\pm$0.21 \\
    LightPath w/o pretrain & 50.17$\pm$0.87 & 84.01$\pm$1.23 & 17.91$\pm$0.89 & 17.03$\pm$0.81 & 28.19$\pm$1.82 & 58.52$\pm$3.79 & 5.09$\pm$0.9 & 3.67$\pm$0.74 \\
    LightPath & 55.99$\pm$0.04 & 88.65$\pm$0.23 & 23.04$\pm$0.28 & 21.23$\pm$0.6 & 33.51$\pm$0.96 & 66.94$\pm$1.52 & 8.06$\pm$0.56 & 7.2$\pm$0.48 \\
    \bottomrule
    \end{tabular}
}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}

==> table/destination_v1.tex <==
\begin{threeparttable}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|cccc|cccc}
    \toprule
    \multirow{2}{*}{Method} & \multirow{2}{*}{Mode} &\multicolumn{4}{c|}{Chengdu} & \multicolumn{4}{c}{Porto} \\ 
    % \cmidrule(lr){3-6} \cmidrule(lr){7-10}
    \cline{3-10}
    %\cmidrule{3-10}
    & & Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) & 
    Acc@1(\%) & Acc@5(\%) & Recall(\%) & f1(\%) \\
    \midrule
    \multirow{3}{*}{CAESC} 
    & w/o finetune & 18.55$\pm$0.7 & 50.35$\pm$1.37 & 4.73$\pm$0.82 & 3.23$\pm$0.63 & 15.99$\pm$1.33 & 36.19$\pm$2.51 & 1.75$\pm$0.31 & 1.04$\pm$0.22\\
    & w/o pretrain & 24.38$\pm$4.31 & 60.5$\pm$5.38 & 7.07$\pm$1.86 & 5.22$\pm$1.77 & 34.2$\pm$3.56 & 67.22$\pm$5.95 & 8.91$\pm$3.16 & 7.7$\pm$3.23\\
    & full & 16.71$\pm$2.28 & 43.17$\pm$5.66 & 2.59$\pm$0.98 & 1.43$\pm$0.68 & 28.74$\pm$2.22 & 58.29$\pm$4.12 & 4.71$\pm$0.93 & 3.46$\pm$0.96 \\
    \midrule
    \multirow{3}{*}{GCM} 
    & w/o finetune & 53.73$\pm$0.3 & 86.56$\pm$0.21 & 22.45$\pm$0.83 & 20.85$\pm$0.85 & 33.43$\pm$0.41 & 66.74$\pm$0.41 & 8.16$\pm$0.26 & 7.36$\pm$0.34\\
    & w/o pretrain & 54.64$\pm$0.38 & 87.59$\pm$0.23 & 22.79$\pm$1.12 & 20.96$\pm$0.99 & 34.29$\pm$0.26 & 68.05$\pm$0.14 & 8.61$\pm$0.44 & 7.61$\pm$0.55\\
    & full & 54.88$\pm$0.27 & 87.59$\pm$0.11 & 23.03$\pm$0.45 & 21.21$\pm$0.52 & 34.43$\pm$0.47 & 68.51$\pm$0.26 & 8.95$\pm$0.36 & 8.05$\pm$0.44 \\
    \midrule
    \multirow{3}{*}{GM-VSAE} 
    & w/o finetune & 31.85$\pm$0.4 & 70.07$\pm$0.28 & 15.04$\pm$1.69 & 13.85$\pm$1.73 & 24.43$\pm$0.3 & 49.36$\pm$0.21 & 6.24$\pm$0.26 & 5.89$\pm$0.19\\
    & w/o pretrain & 38.96$\pm$0.63 & 80.82$\pm$0.73 & 18.67$\pm$0.68 & 16.53$\pm$0.96 & 43.76$\pm$0.22 & 79.41$\pm$0.27 & 14.73$\pm$0.21 & 13.82$\pm$0.42\\
    & full & 39.25$\pm$0.24 & 80.67$\pm$0.16 & 18.91$\pm$0.52 & 16.96$\pm$0.73 & 43.7$\pm$0.36 & 79.04$\pm$0.16 & 14.68$\pm$0.26 & 13.69$\pm$0.35\\
    \midrule
    \multirow{3}{*}{PreCLN} 
    & w/o finetune & 12.48$\pm$0.2 & 31.92$\pm$0.12 & 2.26$\pm$1.02 & 2.09$\pm$1.02 & 9.58$\pm$0.19 & 24.79$\pm$0.29 & 0.62$\pm$0.01 & 0.34$\pm$0.02\\
    & w/o pretrain & 53.06$\pm$0.51 & 87.63$\pm$0.39 & 20.33$\pm$0.59 & 18.03$\pm$0.73 & 37.35$\pm$0.19 & 73.14$\pm$0.12 & 9.96$\pm$0.23 & 8.66$\pm$0.24\\
    & full & 48.45$\pm$1.24 & 83.9$\pm$1.41 & 14.55$\pm$1.63 & 11.58$\pm$1.54 & 36.5$\pm$0.28 & 72.0$\pm$0.5 & 8.99$\pm$0.13 & 7.46$\pm$0.18 \\
    \midrule
    \multirow{3}{*}{START} 
    & w/o finetune & 47.21$\pm$0.26 & 79.72$\pm$0.25 & 18.31$\pm$1.29 & 17.13$\pm$1.61 & 28.92$\pm$0.19 & 59.12$\pm$0.27 & 6.35$\pm$0.17 & 5.63$\pm$0.31\\
    & w/o pretrain & 55.14$\pm$1.91 & 87.83$\pm$1.14 & 21.46$\pm$3.23 & 19.14$\pm$3.73 & 36.13$\pm$0.69 & 71.33$\pm$0.94 & 9.17$\pm$0.59 & 7.63$\pm$0.64\\
    & full & 55.28$\pm$0.81 & 86.53$\pm$2.5 & 23.81$\pm$3.7 & 21.84$\pm$4.44 & 36.87$\pm$0.33 & 72.96$\pm$0.31 & 9.96$\pm$0.41 & 8.41$\pm$0.4\\
    \midrule
    \multirow{3}{*}{TremBR} 
    & w/o finetune & 22.44$\pm$0.63 & 48.91$\pm$1.16 & 3.4$\pm$0.78 & 2.56$\pm$0.72 & 4.89$\pm$0.46 & 13.68$\pm$0.45 & 0.14$\pm$0.02 & 0.03$\pm$0.02\\
    & w/o pretrain & 57.86$\pm$0.24 & 90.27$\pm$0.18 & 25.64$\pm$0.3 & 23.87$\pm$0.24 & 38.5$\pm$0.52 & 75.31$\pm$0.31 & 11.03$\pm$0.4 & 9.5$\pm$0.53\\
    & full & 56.09$\pm$0.19 & 88.4$\pm$0.27 & 23.88$\pm$0.6 & 22.06$\pm$0.67 & 38.14$\pm$0.16 & 74.16$\pm$0.31 & 10.14$\pm$0.24 & 8.6$\pm$0.26\\
    \midrule
    \multirow{3}{*}{TrajectorySim} 
    & w/o finetune & 30.42$\pm$0.31 & 57.10$\pm$0.30 & 8.33$\pm$0.83 & 8.29$\pm$0.99 & 19.42$\pm$0.27 & 43.07$\pm$0.28 & 2.60$\pm$0.10 & 2.22$\pm$0.10\\
    & w/o pretrain & 34.22$\pm$0.23 & 60.20$\pm$0.32 & 10.93$\pm$0.32 & 11.29$\pm$0.19 & 22.90$\pm$0.37 & 49.23$\pm$0.21 & 3.49$\pm$0.13 & 3.02$\pm$0.23\\
    & full & 33.48$\pm$0.35 & 60.32$\pm$0.26 & 9.30$\pm$0.57 & 9.51$\pm$0.68 & 22.36$\pm$0.08 & 48.23$\pm$0.20 & 3.25$\pm$0.12 & 2.77$\pm$0.12\\
    \midrule
    \multirow{3}{*}{t2vec} 
    & w/o finetune & 54.47$\pm$0.28 & 86.80$\pm$0.17 & 24.41$\pm$0.98 & 22.84$\pm$1.13 & 37.81$\pm$0.26 & 72.82$\pm$0.20 & 10.27$\pm$0.25 & 9.44$\pm$0.28\\
    & w/o pretrain & 55.67$\pm$0.21 & 87.71$\pm$0.24 & 24.96$\pm$0.70 & 23.29$\pm$0.77 & 38.14$\pm$0.25 & 73.76$\pm$0.27 & 10.70$\pm$0.49 & 9.29$\pm$0.67\\
    & full & 55.63$\pm$0.29 & 88.16$\pm$0.08 & 24.25$\pm$0.97 & 22.15$\pm$1.17 & 38.71$\pm$0.29 & 74.35$\pm$0.50 & 10.83$\pm$0.28 & 9.77$\pm$0.17\\
    \midrule
    \multirow{3}{*}{RobustDAA} 
    & w/o finetune & 5.84$\pm$0.03 & 15.74$\pm$2.41 & 0.11$\pm$0.001 & 0.01$\pm$0.002 & 4.88$\pm$0.07 & 14.27$\pm$0.17 & 0.21$\pm$0.01 & 0.04$\pm$0.004\\
    & w/o pretrain & 8.13$\pm$0.62 & 20.10$\pm$1.87 & 0.50$\pm$0.21 & 0.42$\pm$0.21 & 5.54$\pm$0.13 & 14.81$\pm$1.05 & 0.31$\pm$0.05 & 0.22$\pm$0.05\\
    & full & 5.84$\pm$0.06 & 16.59$\pm$0.98 & 0.11$\pm$0.001 & 0.01$\pm$0.002 & 5.76$\pm$0.22 & 16.77$\pm$0.36 & 0.31$\pm$0.05 & 0.15$\pm$0.05\\
    \midrule
    \multirow{3}{*}{trajectory2vec} 
    & w/o finetune & 26.57$\pm$0.28 & 53.52$\pm$0.12 & 3.99$\pm$0.28 & 3.66$\pm$0.09 & 8.25$\pm$0.21 & 21.17$\pm$0.23 & 0.46$\pm$0.03 & 0.22$\pm$0.02\\
    & w/o pretrain & 29.35$\pm$1.43 & 56.97$\pm$1.68 & 4.68$\pm$0.37 & 4.15$\pm$0.35 & 4.92$\pm$0.10 & 13.50$\pm$0.25 & 0.14$\pm$0.01 & 0.03$\pm$0.01\\
    & full & 36.25$\pm$1.20 & 64.99$\pm$1.59 & 7.55$\pm$1.02 & 6.99$\pm$1.03 & 6.07$\pm$1.72 & 15.96$\pm$4.63 & 0.39$\pm$0.05 & 0.16$\pm$0.05\\
    \midrule
    \multirow{3}{*}{DTC} 
    & w/o finetune & 6.56$\pm$0.66 & 16.86$\pm$0.55 & 0.13$\pm$0.02 & 0.03$\pm$0.01 & 4.02$\pm$1.16 & 10.29$\pm$2.65 & 0.12$\pm$0.00 & 0.01$\pm$0.00\\
    & w/o pretrain & 55.43$\pm$0.27 & 87.87$\pm$0.25 & 23.56$\pm$1.10 & 21.40$\pm$1.18 & 38.26$\pm$0.28 & 73.72$\pm$0.18 & 10.53$\pm$0.19 & 8.84$\pm$0.13\\
    & full & 54.69$\pm$0.36 & 86.44$\pm$0.30 & 23.31$\pm$0.42 & 21.27$\pm$0.49 & 36.02$\pm$0.14 & 70.86$\pm$0.41 & 8.90$\pm$0.22 & 7.87$\pm$0.13\\
    \midrule
    \multirow{3}{*}{LightPath} 
    & w/o finetune & 51.0$\pm$0.20 & 84.11$\pm$0.23 & 18.62$\pm$0.59 & 16.72$\pm$0.64 & 31.48$\pm$0.11 & 63.55$\pm$0.09 & 7.16$\pm$0.23 & 6.36$\pm$0.21 \\
    & w/o pretrain & 50.17$\pm$0.87 & 84.01$\pm$1.23 & 17.91$\pm$0.89 & 17.03$\pm$0.81 & 28.19$\pm$1.82 & 58.52$\pm$3.79 & 5.09$\pm$0.9 & 3.67$\pm$0.74 \\
    & full & 55.99$\pm$0.04 & 88.65$\pm$0.23 & 23.04$\pm$0.28 & 21.23$\pm$0.6 & 33.51$\pm$0.96 & 66.94$\pm$1.52 & 8.06$\pm$0.56 & 7.2$\pm$0.48 \\
    \bottomrule
    \end{tabular}
}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}

==> table/finetune-scalability.tex <==
\begin{threeparttable}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    Scale & \multicolumn{6}{c}{20\%/40\%/60\%/80\%} \\
    \midrule
    Datasets & \multicolumn{3}{c|}{Chengdu} & \multicolumn{3}{c}{Porto} \\
    \midrule
    Metric & Acc@1(\%) & Recall(\%) & f1(\%) & Acc@1(\%) & Recall(\%) & f1(\%) \\
    \midrule
    CAESC & 100.0/99.7/100.0/100.0 & 100.0/49.9/100.0/100.0 & 100.0/49.9/100.0/100.0 & 98.2/99.4/98.8/98.8 & 78.6/79.8/79.0/98.8 & 79.3/79.8/79.5/99.3 \\
    \bottomrule
    \end{tabular}
}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}

==> table/pretrain-scalability.tex <==
\begin{threeparttable}
\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    Scale & \multicolumn{6}{c}{20\%/40\%/60\%/80\%} \\
    \midrule
    Datasets & \multicolumn{3}{c|}{Chengdu} & \multicolumn{3}{c}{Porto} \\
    \midrule
    Metric & Acc@1(\%) & Acc@5(\%) & Acc@10(\%) & Acc@1(\%) & Acc@5(\%) & Acc@10(\%) \\
    \midrule
    CAESC & & & & & & \\
    TrajectorySim & 84.7/96.2/108.0/93.9 & 97.9/105.5/108.9/104.9 & 95.8/102.8/105.3/102.2 & 101.0/103.1/109.9/106.8 & 101.1/104.7/109.4/107.2 & 104.7/108.1/108.1/109.8 \\
    t2vec & 102.0/101.2/100.6/100.0 & 101.4/101.2/101.1/101.2 & 100.8/100.6/100.6/100.3 & 100.8/99.8/100.2/100.4 & 100.4/100.8/100.2/100.6 & 99.8/99.8/99.6/99.6 \\
    RobustDAA & 100.0/100.2/100.0/100.0 & 99.8/100.4/99.8/99.8 & 100.9/101.5/100.0/99.1 & 100.0/100.4/100.0/100.0 & 99.3/100.4/99.6/98.9 & 99.6/100.4/100.4/98.9 \\
    DTC & 61.2/64.2/75.9/ 87.5 & 
    68.2/71.0/81.6/90.8 & 
    70.7/75.3/86.7/95.3 & 
    134.7/112.2/120.4/112.2 &
    118.1/108.3/112.5/95.8 & 116.0/111.1/122.2/103.7 \\
    trajectory2vec & 
    36.7/56.7/56.7/66.7 &
    36.7/54.4/77.8/73.3 & 
    45.3/71.8/85.5/80.3 &
    88.9/100.0/88.9/111.1 & 
    104.5/86.4/109.1/90.9 & 
    105.6/88.9/102.8/111.1\\
    % CAESC & 100.0/99.7/100.0/100.0 & 100.0/49.9/100.0/100.0 & 100.0/49.9/100.0/100.0 & 98.2/99.4/98.8/98.8 & 78.6/79.8/79.0/98.8 & 79.3/79.8/79.5/99.3 \\
    % GCM & 96.8/98.5/99.4/99.6 & 22.3/42.2/59.6/81.2 & 22.7/42.5/59.8/80.3 & 98.8/98.8/99.4/99.4 & 59.3/59.3/74.6/74.6 & 59.6/59.6/74.8/74.8 \\
    % GM-VSAE & 26.0/54.6/69.3/86.0 & 2.8/11.9/26.9/37.6 & 4.3/15.4/31.7/40.4 & 62.0/80.2/84.2/92.3 & 17.4/53.4/46.3/73.8 & 19.4/54.1/46.0/70.4 \\
    % PreCLN &  & & & & & \\
    % START & 52.6/78.0/92.3/96.7 & 1.9/4.0/6.3/8.1 & 2.7/4.9/7.1/9.0 & 70.8/86.2/94.9/96.1 & 10.4/30.7/53.7/56.4 & 11.7/31.9/54.5/57.4 \\
    % TremBR & 138.4/117.1/83.5/95.7 & 202.7/141.2/66.5/93.4 & 180.3/133.8/70.2/94.7 & 153.3/114.4/116.7/98.9 & 396.9/111.9/155.6/114.5 & 335.4/106.6/147.1/114.9 \\
    % TrajectorySim & 73.6/104.6/87.4/94.3 & 76.5/111.0/84.1/108.9 & 80.8/110.0/86.3/110.2 & 76.6/112.5/112.5/120.3 & 66.6/123.0/123.0/152.8 & 71.2/118.9/118.9/144.9 \\
    % t2vec & 100.9/100.9/101.8/100.3 & 185.0/158.6/224.0/122.6 & 184.2/157.9/222.0/122.4 & 100.6/100.0/101.2/101.8 & 167.7/83.3/168.7/169.7 & 167.2/83.3/167.7/168.2 \\
    % RobustDAA & 100.0/100.0/100.7/100.0 & 100.0/103.6/99.0/100.0 & 100.0/103.6/98.8/100.0 & 101.1/100.0/100.0/100.0 & 106.9/105.7/100.0/100.0 & 106.5/105.7/100.0/100.0 \\
    % LightPath & 84.8/96.2/96.5/98.8 & 7.9/22.2/41.3/49.4 & 8.6/22.6/42.1/49.7 & 95.8/97.0/97.6/99.4 & 34.8/48.5/65.1/66.3 & 35.6/49.2/65.8/66.5 \\
    \bottomrule
    \end{tabular}
}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}

==> table/similar.tex <==
\begin{threeparttable}
%\resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|ccc|ccc}
    \toprule
    Datasets & \multicolumn{3}{c|}{Chengdu} & \multicolumn{3}{c}{Porto} \\
    \midrule
    Metric & Acc@1(\%) & Acc@5(\%) & Acc@10(\%) & 
    Acc@1(\%) & Acc@5(\%) & Acc@10(\%) \\
    \midrule
    CAESC & 99.77 & 99.77 & 99.77 & 95.93  & 96.51  & 96.51 \\
    TrajectorySim & 25.29 & 31.69 & 34.88 & 37.21 & 53.49 & 57.56 \\
    t2vec & 97.09 & 98.26 & 99.13 & 97.09 & 98.26 & 99.42 \\
    RobustDAA & 43.31 & 43.60 & 43.90 & 52.33 & 52.91 & 52.91\\
    DTC & 22.48 & 27.42 & 29.07 & 9.50 & 13.95 & 15.70 \\
    trajectory2vec & 2.91 & 8.72 & 11.34 & 1.74 & 4.26 & 6.98\\
    GCM & 98.55  & 98.84  & 98.84 & 99.07 & 99.41 & 99.41 \\
    GM-VSAE & 86.34  & 92.44  & 93.31  & 65.69 & 71.51 & 73.26 \\
    % PreCLN & 0.58  & 0.87  & 0.0  & 0.0  & 1.16  & 1.16  & 0.01  & 0.01 \\
    PreCLN & 54.07 & 61.05 & 64.53 & 48.55 & 55.52 & 58.43 \\
    START & 68.31 & 80.23 & 84.96 & 66.86 & 79.65 & 83.63 \\
    TremBR & 53.48 & 60.76 & 63.95 & 59.30 & 66.28 & 69.18\\
    % TrajectorySim & 25.29 & 31.40 & 0.49 & 0.78 & 37.21 & 53.49 & 0.79  & 1.15\\
    % t2vec & 97.09 & 98.26 & 8.83 & 8.96 & 97.09 & 98.26 & 19.42  & 19.71\\
    % RobustDAA & 43.31 & 43.60 & 0.75 & 1.04 & 52.33 & 50.00 & 1.41  & 1.86\\
    % DTC & 2.62 & 6.10 & 0.01 & 0.02 & 1.16 & 2.91 & 0.01  & 0.01\\
    % trajectory2vec & 3.78 & 9.01 & 0.02 & 0.03 & 1.16 & 3.49 & 0.01  & 0.01\\
    LightPath & 97.97 & 99.13 & 99.71 & 96.51 & 97.67 & 97.67 \\
    \bottomrule
    \end{tabular}
%}
    \begin{tablenotes}\footnotesize
        \item[]{\textbf{Bold} denotes the best result, 
        \underline{underline} denotes the second best result.}
    \end{tablenotes}
\end{threeparttable}
